Lexical Features in Coreference Resolution: To be Used With Caution

Lexical features are a major source of information in state-of-the-art coreference resolvers. Lexical features implicitly model some of the linguistic phenomena at a fine granularity level. They are especially useful for representing the context of mentions. In this paper we investigate a drawback of using many lexical features in state-of-the-art coreference resolvers. We show that if coreference resolvers mainly rely on lexical features, they can hardly generalize to unseen domains. Furthermore, we show that the current coreference resolution evaluation is clearly flawed by only evaluating on a specific split of a specific dataset in which there is a notable overlap between the training, development and test sets.

==> exp.tex <==
\section{Evaluations on the New Split}



\begin{table*}[t]
    \begin{center}\footnotesize
    \resizebox{2\columnwidth}{!}{%
    \begin{tabular}{l|rrr|rrr|rrr|r||rrr}
     \multicolumn{1}{c}{} & \multicolumn{3}{c}{MUC} &
     \multicolumn{3}{c}{$B^3$} & \multicolumn{3}{c}{CEAF$_e$} & CoNLL & \multicolumn{3}{c}{LEA} \\ \hline
     \multicolumn{1}{c|}{}&R & P & F$_1$ & R & P & F$_1$ & R & P & F$_1$ & Avg. F$_1$ & R & P & F$_1$\\
         \multicolumn{1}{c|}{} & \multicolumn{13}{c}{Official Split} \\ \hline
     \hline
     dcoref & $64.29$ & $65.19$ & $64.74$ & $49.18$ & $56.79$ & $52.71$ & $52.45$ & $46.58$ & $49.34$ & $55.60$ & $43.72$ & $51.53$ & $47.30$ \\
     berkeley & $67.15$ & $72.1$ & $69.54$ & $52.06$ & $60.04$ & $55.77$ & $51.35$  & $54.69$ & $52.97$ & $59.43$ & $47.38$ & $55.47$ & $51.11$ \\
      cort  & $67.83$ & $78.35$ & $72.71$ & $54.34$ & $68.42$ & $60.57$ & $53.10$ & $61.10$ & $56.82$ & $63.37$ & $50.40$ & $64.46$ &$56.57$\\ %& $74.92$ & $84.64$ & $79.48$
      %deep-coref & $69.05$ & $80.93$ & $74.52$ & $56.30$ & $71.80$ & $63.11$ & $53.81$ & $64.50$ & $58.68$ & $65.44$ & $52.77$ & $68.27$ & $59.53$ \\ 
	  deep-coref & $69.38$ & $80.68$ & $74.6$ & $56.78$ & $71.60$ & $63.34$ & $53.89$ & $64.63$ & $58.78$ & $65.57$& $53.28$& $68.18$ & $59.82$ \\
	  \hline
    \multicolumn{1}{c|}{} & \multicolumn{13}{c}{-TC} \\ \hline
	dcoref & $63.54$ & $64.95$ & $64.23$ & $48.56$ & $56.66$ & $52.3$ & $52.4$ & $47.01$ & $49.56$ & $55.36$& $43.04$ & $51.26$ & $46.79$ \\
	berkeley & $66.34$ & $71.3$ & $68.73$ & $51.4$ & $60.34$ & $55.51$ & $51.59$ & $54.77$ & $53.13$ & $59.12$&$46.57$ & $55.65$ & $50.71$\\
	cort & $67.1$ & $77.82$ & $72.06$ & $53.58$ & $68.54$ & $60.14$ & $53.54$ & $61.19$ & $57.11$ & $63.10$& $49.51$ & $64.44$ & $56$\\
	deep-coref& $68.8$ & $80.06$ & $74.00$ & $56.13$ & $71.2$& $62.77$ & $54.25$ & $64.6$ & $58.97$ & $65.24$ & $52.51$ & $67.64$ & $59.12$ \\
    \multicolumn{1}{c|}{} & \multicolumn{13}{c}{New Split} \\ \hline
    \hline
     dcoref & $60.26$ & $62.02$ & $61.13$ & $46.39$ & $54.53$ & $50.13$ & $51.10$ & $44.9$ & $47.80$ & $53.02$ & $40.51$ & $48.66$ & $44.21$ \\
     %cort+sing & $58.82$ & $78.59$ & $67.28$ & $44.85$ & $72.08$ & $55.3$ & $49.27$ & $57.19$ & $52.94$ &  $58.51$ & $40.84$ & $67.71$ & $50.95$\\
     berkeley & $61.78$ & $69.78$ & $65.54$ & $46.92$ & $59.22$ & $52.36$ & $48.03$ & $52.15$ & $50.01$ & $55.97$ & $41.94$ & $54.03$ & $47.23$\\
     cort & $63.19$ & $75.78$ & $68.92$ & $49.92$ & $66.89$ & $57.17$ & $50.60$ & $57.88$ & $54.00$ & $60.03$ & $45.65$ & $62.41$ & $52.73$ \\
     deep-coref & $64.66$ & $76.98$ & $70.28$ & $51.65$ &$67.83$ & $58.65$ &  $51.10$ &$60.37$ & $55.35$ & $61.43$ & $47.68$ &$63.66$ & $54.52$ \\
     \multicolumn{1}{c|}{} & \multicolumn{13}{c}{Newer! Split} \\ \hline
     dcoref & $64.36$ & $64.45$ & $64.41$ & $49.71$ & $56.6$ & $52.93$ & $53.47$ & $46.01$ & $49.46$ & $55.6$ & $43.86$ & $50.95$ & $47.14$\\

    \end{tabular}
    }
    \end{center}
    \caption{Results on the test sets.}
    \label{tab:real_data}
\end{table*}
\begin{table}[t]
    \begin{center}\footnotesize
    \begin{tabular}{rrrrrrr}
     bc & bn & mz & nw & pt & tc & wb \\ \hline
     \multicolumn{7}{c}{train+dev} \\ \hline
     $33\%$ & $42\%$ & $47\%$ & $38\%$ & $76\%$ & $36\%$ & $33\%$\\ \hline
      \multicolumn{7}{c}{train} \\ \hline
     $25\%$ & $40\%$ & $47\%$ & $35\%$ & $75\%$ & $34\%$ & $29\%$\\
    \end{tabular}
    \end{center}
    \caption{Non-pronominal coreferent mentions that are always coreferent in the training data.}
    \label{tab:new_split_coref_ratio}
\end{table}
%
\begin{table}[t]
    \begin{center}\footnotesize
    \begin{tabular}{l|rrrrrrr}
     \multicolumn{1}{c|}{} & I & you & he & she & it & we & they \\ \hline
     \multicolumn{1}{c}{} & \multicolumn{7}{c}{Recall errors} \\ \hline
     dcoref & $95$ & $197$ & $316$ & $96$ & $488$ & $144$ & $527$\\
     deep-coref & $69$ & $196$ & $186$ & $58$ & $466$ & $123$ & $338$\\
     \multicolumn{1}{c}{} & \multicolumn{7}{c}{Precision errors} \\ \hline
     dcoref & $209$ & $462$ & $362$ & $77$ & $992$ & $282$ & $556$\\
     deep-coref& $112$ & $224$ & $165$ & $57$ & $287$ & $147$ & $381$\\
    \end{tabular}
    \end{center}
    \caption{Error analysis for different pronouns on the CoNLL 2012 development set.}
    \label{tab:pronoun_error}
\end{table}

\begin{table}[t]
    \begin{center}\footnotesize
 %   \resizebox{2\columnwidth}{!}{%
    \begin{tabular}{l|r|r}
     \multicolumn{1}{c}{} & \multicolumn{1}{c}{Anaphoric} &
     \multicolumn{1}{c}{Non-anaphoric}\\ \hline
    \hline
	\multicolumn{1}{c}{} & \multicolumn{1}{c}{it} \\ \hline
	gold & $468$ & $881$\\
	dcoref & $132$\\
	deep-coref& $562$\\
	\multicolumn{1}{c}{} & \multicolumn{1}{c}{they} \\ \hline
	gold & \\
	dcoref & \\
	deep-coref& \\
	 
    \end{tabular}
  %  }
    \end{center}
    \caption{Error analysis for pronouns it and they.}
    \label{tab:real_data}
\end{table}

\begin{table*}[t]
    \begin{center}\footnotesize
 %   \resizebox{2\columnwidth}{!}{%
    \begin{tabular}{l|r|r|r|r||r}
     \multicolumn{1}{c}{} & \multicolumn{1}{c}{MUC} &
     \multicolumn{1}{c}{$B^3$} & \multicolumn{1}{c}{CEAF$_e$} & CoNLL & \multicolumn{1}{c}{LEA} \\ \hline
    \hline
     deep-coref  &  $70.08$ & $60.53$ & $57.72$ & $62.78$ & $56.23$  \\
     -avg. embeddings  & $69.84$ & $60.53$ & $57.48$ & $62.61$  & $56.23$ \\
     -genre & \\
    \end{tabular}
  %  }
    \end{center}
    \caption{Results on the new dev set.}
    \label{tab:real_data}
\end{table*}

\begin{table}[t]
    \begin{center}\footnotesize
 %   \resizebox{2\columnwidth}{!}{%
    \begin{tabular}{l|rrr}
	 \multicolumn{1}{c}{} &	\multicolumn{3}{c}{Anaphor} \\
     \multicolumn{1}{c}{} & Proper & Nominal & Pronominal \\ \hline
	 \multicolumn{1}{c}{Antecedent} & \multicolumn{3}{c}{Correct decisions} \\ \hline
	 Proper & $193$ & $23$ & $100$\\
	 Nominal & $3$ & $120$ & $136$ \\
	 Pronominal & $6$ & $19$ & $748$\\
	 \hline
	 \multicolumn{1}{c}{} & \multicolumn{3}{c}{Correct decisions} \\ \hline
	 Proper & $1632$ & $45$ & $500$\\
	 Nominal & $14$ & $463$ & $426$\\
	 Pronominal & $18$ & $32$ &  \\
	 \hline
    \end{tabular}
  %  }
    \end{center}
    \caption{Number of pairwise decisions made by deep-coref for which an exact pair was seen in the training data.}
    \label{tab:deep_coref_made_decisions}
\end{table}



\begin{table}[t]
    \begin{center}\footnotesize
 %   \resizebox{2\columnwidth}{!}{%
    \begin{tabular}{ll|rrr}
	 \multicolumn{2}{c}{} &	\multicolumn{3}{c}{Anaphor} \\
     \multicolumn{1}{c}{Antecedent} & & \multicolumn{1}{c}{Proper} & \multicolumn{1}{c}{Nominal} & \multicolumn{1}{c}{Pronominal} \\ \hline
	 \multirow{2}{*}{Proper} 
	 &seen & $53\%$ & $38\%$ & $48\%$\\
	 &all & $3307$ & $197$ & $1220$\\
	  \hline
	 \multirow{2}{*}{Nominal} 
	 &seen & $80\%$ & $93\%$ & $93\%$\\
	 &all & $25$ & $1599$ & $1451$\\
	  \hline
	 \multirow{2}{*}{Pronominal}
	  & seen & $68\%$ & $100\%$ & $100\%$\\
	  & all &  $38$ & $24$ & $4919$\\
	 \hline
    \end{tabular}
  %  }
    \end{center}
    \caption{Number of pairwise decisions made by cort for which the head-pair was seen in the training data.}
    \label{tab:deep_coref_made_decisions}
\end{table}
\begin{table*}[t]
    \begin{center}\footnotesize
 %   \resizebox{2\columnwidth}{!}{%
    \begin{tabular}{l|rrrr}
     \multicolumn{1}{c}{} & Proper & Nominal & Pronominal & List \\ \hline
	 \multicolumn{1}{c}{} & \multicolumn{1}{c}{Correct decisions} \\ \hline
	 Proper & \\
	 Nominal & \\
	 Pronominal & \\
	 List & \\ \hline
	 \multicolumn{1}{c}{} & \multicolumn{1}{c}{Correct decisions} \\ \hline
	 Proper & \\
	 Nominal & \\
	 Pronominal & \\
	 List & \\ \hline
    \end{tabular}
  %  }
    \end{center}
    \caption{Pairwise decisions made by cort.}
    \label{tab:deep_coref_made_decisions}
\end{table*}




==> extra.tex <==
\begin{table}[t]
    \begin{center}\footnotesize
 %   \resizebox{2\columnwidth}{!}{%
    \begin{tabular}{ll|rrr}
	 \multicolumn{2}{c}{} &	\multicolumn{3}{c}{Anaphor} \\
     \multicolumn{1}{c}{Antecedent} & & \multicolumn{1}{c}{Proper} & \multicolumn{1}{c}{Nominal} & \multicolumn{1}{c}{Pronominal} \\ \hline
	 \multirow{2}{*}{Proper} 
	 &seen & $80\%$ & $51\%$ & $79\%$ \\ 
	 &all & $3655$ & $323$  & $1351$ \\ 
	  \hline
	 \multirow{2}{*}{Nominal} 
	 &seen & $59\%$ & $90\%$ & $94\%$ \\
	 &all & $139$ & $2131$ & $2141$ \\
	  \hline
	 \multirow{2}{*}{Pronominal}
	  & seen & $78\%$ & $92\%$ & $100\%$\\
	  & all & $191$ & $250$ & $4966$\\
	 \hline
    \end{tabular}
  %  }
    \end{center}
    \caption{Number of links created by rule-based for which the head-pair exists in the training data.}
    \label{tab:dcoref_head_seen}
\end{table}

==> wikicoref.tex <==
\section{Out of Domain Evaluation}

